Reinforcement Learning and Adaptive Sampling for Optimized DNN Compilation

Achieving faster execution with shorter compilation time can enable further diversity and innovation in neural networks. However, the current paradigm of executing neural networks either relies on hand-optimized libraries, traditional compilation heuristics, or very recently, simulated annealing and genetic algorithms. Our work takes a unique approach by formulating compiler optimizations for neural networks as a reinforcement learning problem, whose solution takes fewer steps to converge. This solution, dubbed ReLeASE, comes with a sampling algorithm that leverages clustering to focus the costly samples (real hardware measurements) on representative points, subsuming an entire subspace. Our adaptive sampling not only reduces the number of samples, but also improves the quality of samples for better exploration in shorter time. As such, experimentation with real hardware shows that reinforcement learning with adaptive sampling provides 4.45x speed up in optimization time over AutoTVM, while also improving inference time of the modern deep networks by 5.6%. Further experiments also confirm that our adaptive sampling can even improve AutoTVM's simulated annealing by 4.00x.

==> figs/bsplot/.git/objects/03/c63510ec5749ecf759fe42c0f10023fc909b92 <==
x•"Ánâ0†÷œ§˜›A5ZÚJ8잨¶*U/(ŠL2´Q%%o¿3v ­šŠg~ó{âxkö[P¥~ey±/k¨š* +,týê¢@›DŠaÐ
Lf1RÜA®3;Þ@¿Ó8Ã6c	·ԍ"ÉLÂt"a6Žœ¢éôtJ	×n|"æ«ïæ"ôöÂ8«"xÆ\ÂܼÕï¥etQšMF©ÍeëBõ»¸Ì<g'ûäÝÛ÷9'ý9yýìŸÄœj֒:5{ÿÐHHí®µ3é·ó-ôlï¼*F{bõv§?²Û©­FQí½Ã¯Wk{ú#۝ڻ½#ò—,žì½ó>Ùð†"¼íT$as¢—J#z}nDå¥UύÈ=(MÔVßx?J Þ‰ Þ iPX#CÄ:ËFטÂÒZÔôm¼Âàùåa($ˆ'Ììn_&˜£­a…º´çHß´+X¦º¨³#ÂZç£>B>1à
úƒ'\árý{(¢À•Ê8"£ƒî¹…Ü‹\8qáÙÿãç%¦ü÷Z"Z¾Ùš^Pôه…Ù׃U×@''òñ­©²Dx@]J·âŠÏV×twª³ä=ÎlåQ›íÇæóú+}ąà&,Ò9A¶ƒ8æLq‹ˆ8æC'Ž…?uü	ü¤&–

==> figs/bsplot/.git/objects/0b/db66ac66fbaff3960ecd6af6495c7ab6d9ddd3 <==
x…ÝJÄ0…½ÎSÌ]Z®[XÈ[x§Ò6Õ`›†$]ÄwwÚZñF6ÌÀ"ùæp8u?ÖPª;ø1$ˆ92jáuzÚ{ãڂÁK¶NɶÿÝ4ø:'󌵦ƒA[W"gôfð|D¸E8!Tw÷¯+¯ñ R ")*'ª6…U&n¦"ïÇTÌ!"žlo^'™SœêØëÓçüÅÿÙäeC°|
"A˜"m>TÐîÍHç…^§â€p\ºÜë(‹î%¹Ê×N6àïIÔ#ù¯ÿ¶£¤™í@)§£H	\©%T¥ø–ê–0û!ªƒ

==> figs/bsplot/.git/objects/16/82045c39cec103c7b2c193ce81cc56165c4bf3 <==
xÎAnà @Ñ®9Å\ ƒ)ª'®z
<3ؑˆ\¼èíkõÝüå×ãþ|> ¥·±«M3:Ê)ãDdC(jƒdEÅJ©‰CuÎgk^e×6`¢˜Ð±¯I™£g>ëôR³&œ£)ÇXûŸ?G[à«÷÷µÁu^ËÚÝMÛr9ø[.*ǸâäÒɂw­5üçúÿƒ)"°é¢M ž'íÑôµõa~NÇLÅ

==> figs/bsplot/.git/objects/5b/613cd042edf136af1819d9c15735a8ad949bfd <==
x-PÁjÄ ìÙ¯x7²Ñn–-ø…ímé¥-ân^¶ÒhĘ%ùûÁyŽÌ¼¹õÃ
"8¿ë‡a\F'.ó:þ2í=º¶ ŒÑ'ì'›"´ØÕÆåtfðE/5­€^xF'ñ5ã1cC²xYŜñ³¨@°Zð
8kxbœšfý<Òà¬>ò͒})™ù~ˆÅ\Á''Ö¥ïևá‰]"4÷z±íêÞ¸×Ϗ2É'g¢¤szÍÑÜÿÔ=Ù0Èk˜°'µÛY¼›ìNFýDIs~Û¥*ˆé@)§-*RUjmC)ºÕ±UCþKQbr

==> figs/bsplot/.git/objects/61/8bd5cc4b18406f10716cad84992f81318832a3 <==
x…ÝJÄ0…½ÎSÌ]Z®Ö"¼…w*!m³LӐ¤KƒøîN[+ÞȆH˜s>&§ucMs¸²Cc†T£Açw¡C0¾¯¸¼f» Ó9›Èö·Ÿ†P@'ð±Þœ`ÐÖWõ#:3Hx>"\#Ü 4·w÷¯« \¤Aˆ@E(*B5aŤm)ܘ«¡ $"ȳuæ%›9§©M]´!Î_üŸIY&N·Æ)²È§8"9ÛîCEíߌôAèõVŽK×»ÀzÊ䬝¤ÝÊ%Ë&økIúl$ÿýE¢¼™=R^F)¸RK´Jñ-Û-gö
ƒ…{

==> figs/bsplot/.git/objects/9b/3dd3b0dce5fd2bd9c975bfabdd5697e4b5062f <==
xÎAn!@Ñ®9…/{RT5]õL¨"@4a½}G=Bwõôóx<¾'óosS…êV©vU²1$]³úD¥°³D	«`Ñ%ºÅ<eÓ>A4EZ+{¶hÉ¥'9—¸p@fô\bB6²Ï66øüÙû
¾Æèpm.©IëDø¡ývÞ󫜵ìï€ÎÇÞQ€"
֚ü÷9õÿ''R û1'›lêQ¯,ó@Ÿ÷1Í/QP

==> figs/bsplot/.git/objects/ae/b92314f46401025bd1614cd9347144164d9b14 <==
xŽQ
!Eûvo
êè¨Q}µ§>g'I¡vŸ´"àü]Î儲m
R™C݉@9¼âRY"âf4܇È-iAÉ:aœ7S'Ñ°'(Ñ뤬ǀcêSG'¢Éï"ȅEå$ÃV—²ÃíÓò÷R2\—'¿à'¥ÊóÐÂ+Û"ÖF½Ã'ÎYøuVúÿaŒPé
‰°¶ Àue_îVM=

==> figs/bsplot/.git/objects/cb/c663e1cedf7c0674605931cc2b873b1aa9ad45 <==
xmQÉnà 홯˜Ž!ÛY*ùc¥ôÒD½´"1IQÍ"Gñß0½‰yÌòތ˜sgÎPçՓTÖô†i@þËÝ7áÖ
Ýf˜¼@©à֛Ñ"Ԋ+(.u¶xAàÏT@Ÿ""y¾JŠº@óU"zƒU"UUœf9›ªém¾ŽP—6›Y¡¤K(½^âDâ£åŽ.Þx	xO£-£­¢­£]áÔé0ùNMA͕ˆ*‡<îåÖÉ»€W¶"úÞ÷ÿfN(Îÿ'Øθ,ŽäµC#AÚӃī²½¹%´ý—¤;îD\kÁC/Ȏo_>jéü𯇓—vñ4Ñ7Ç~ôz7a"à:yÎX=ªäü.œj¯~_H^±0cÐ4€cÏ›·‡~Jæ
